PULSAR: Graph based Positive Unlabeled Learning with Multi Stream Adaptive Convolutions for Parkinson's Disease Recognition

Parkinson's disease (PD) is a neuro-degenerative disorder that affects movement, speech, and coordination. Timely diagnosis and treatment can improve the quality of life for PD patients. However, access to clinical diagnosis is limited in low and middle income countries (LMICs). Therefore, development of automated screening tools for PD can have a huge social impact, particularly in the public health sector. In this paper, we present PULSAR, a novel method to screen for PD from webcam-recorded videos of the finger-tapping task from the Movement Disorder Society - Unified Parkinson's Disease Rating Scale (MDS-UPDRS). PULSAR is trained and evaluated on data collected from 382 participants (183 self-reported as PD patients). We used an adaptive graph convolutional neural network to dynamically learn the spatio temporal graph edges specific to the finger-tapping task. We enhanced this idea with a multi stream adaptive convolution model to learn features from different modalities of data critical to detect PD, such as relative location of the finger joints, velocity and acceleration of tapping. As the labels of the videos are self-reported, there could be cases of undiagnosed PD in the non-PD labeled samples. We leveraged the idea of Positive Unlabeled (PU) Learning that does not need labeled negative data. Our experiments show clear benefit of modeling the problem in this way. PULSAR achieved 80.95% accuracy in validation set and a mean accuracy of 71.29% (2.49% standard deviation) in independent test, despite being trained with limited amount of data. This is specially promising as labeled data is scarce in health care sector. We hope PULSAR will make PD screening more accessible to everyone. The proposed techniques could be extended for assessment of other movement disorders, such as ataxia, and Huntington's disease.

==> Related_Work_OLD.tex <==
Traditional diagnosis methods equipped with the most advanced technologies, play a very important role in Parkinson's disease (PD) diagnosis. Despite recent advances in PD mechanisms, the patient's medical history and physical examinations remain the basis of clinical diagnosis. The clinical diagnosis method is not cost effective and due to that it is very hard to make PD diagnosis accessible for all. 

Machine Learning algorithms have recently been used for PD detection and diagnosis tasks due to their powerful predictive performance.  In the field of PD diagnosis, studies have shown that ML can provide early and reliable diagnosis of patients and help doctors make decisions by analyzing speech, gait or motor tasks.  Therefore, ML algorithms are widely used in both tasks of PD classification and assessment of symptom severity \cite{braga2019automatic,nilashi2020remote,vidya2021gait}. 

In PD classification tasks, a combination of feature selection and machine learning classifiers are used. Senturk \etal \cite{senturk2020early} proposed a prediction model which used recursive feature elimination to select a subset of features and combined it with support vector machines (SVM) to obtain better prediction performance. Govindu \etal \cite{govindu2023early} highlighted the use of machine learning techniques in telemedicine to detect Parkinson’s disease in its early stages. They carried out research on the MDVP audio data of 30 Parkinson’s patients and healthy people during training of 4 ML models. Comparison of results of classification by Support Vector Machine (SVM), Random Forest, K-Nearest Neighbors (KNN) and Logistic Regression models, yield Random Forest classifier as the ideal Machine Learning (ML) technique for detection of Parkinson’s disease. Li \etal \cite{li2022detecting} built a classifier with gait data from Parkinson patients and healthy controls using machine learning methods. The input to their algorithm is the Gait in Parkinson’s Disease dataset published on PhysioNet containing force sensor data as the measurement of gait from 92 healthy subjects and 214 patients with idiopathic Parkinson’s Disease. Different machine learning methods, including logistic regression, SVM, decision tree, KNN were tested to output a predicted classification of Parkinson patients and healthy controls.

Compared with ML techniques, Deep Learning (DL) techniques have attracted a lot of attention because of their powerful automatic feature extraction capabilities \cite{shahid2020deep,srinidhi2021deep}. Sivaranjini \etal \cite{sivaranjini2020deep} developed a deep learning-based approach that classifies PD using Magnetic Resonance (MR) images. Johri \etal \cite{johri2019parkinson} used two separate neural network-based approaches to detect PD. They developed a VGFR spectrogram detector and a voice impairment classifier to detect PD from gait and speech. Guo \etal \cite{guo2022vision} proposed a spatial-temporal 3D hand pose estimation model based on Support Vector Machine to capture and evaluate PD patients’ 3D hand movement. However, the 3D pose still heavily relies on 2D hand pose estimation and introduce extra noises to the hand location, thus in our work, we do not estimate the 3D hand key points. \mdsr{What reference backs your claim of extra noise in 3d pose? Also, the write up suddenly moves from related works to why we do not use 3d pose. It does not feel fluid. For each (or some) of the models from literature, as you introduce them, you could mention their limitations (gap). Then at the end you could mention at the final paragraph of this section how you have decided to cover these gaps.} \msi{In addition to Saifur sir's comment, we can add some relevant papers on PU learning and Graph Neural network in the context of healthcare.}
